Challenging mitosis detection algorithms: Global labels allow centroid localization

Mitotic activity is a crucial proliferation biomarker for the diagnosis and prognosis of different types of cancers. Nevertheless, mitosis counting is a cumbersome process for pathologists, prone to low reproducibility, due to the large size of augmented biopsy slides, the low density of mitotic cells, and pattern heterogeneity. To improve reproducibility, deep learning methods have been proposed in the last years using convolutional neural networks. However, these methods have been hindered by the process of data labelling, which usually solely consist of the mitosis centroids. Therefore, current literature proposes complex algorithms with multiple stages to refine the labels at pixel level, and to reduce the number of false positives. In this work, we propose to avoid complex scenarios, and we perform the localization task in a weakly supervised manner, using only image-level labels on patches. The results obtained on the publicly available TUPAC16 dataset are competitive with state-of-the-art methods, using only one training phase. Our method achieves an F1-score of 0.729 and challenges the efficiency of previous methods, which required multiple stages and strong mitosis location information.

==> sections/3_methods_old.tex <==
\section{Methods}


This section describes the proposed METHOD NAME for automatic mitosis detection in breast cancer histopathology images and the centroid location loss for training the model.

\subsection{Mitosis Classification based on Residual Networks}

\subsubsection{Patching HPFs}

The images used for training and evaluating the model are the HPFs extracted from the H&E WSIs. The size of these HPF varies among the used datasets (SEE FIGURE X). However,  they all correspond to very large images, which cannot be fed directly to a CNN as this would be too computationally demanding for the graphics processing unit (GPU). For this reason, we follow the most common approach in computational pathology for dealing with this problem. Each HPF is cropped into non-overlapping patches, in this case of 500x500 pixels. Therefore, as the provided mitosis centroid coordinates are given with the HPF as a reference, the corresponding masks for each patch are derived, corresponding to a two-dimensional all-zeroes matrix with a positive value in the pixel where the mitosis centroid is located in the analogue H&E patch.

This methodology allows tackling the mitosis detection problem as both a binary patch classification task and a centroid location task. In the first one, the goal is to determine whether a patch contains mitosis, while the second one evaluates the model based on the predicted location of the mitosis in the patch. Therefore, during training, the model is evaluated on both validation and test datasets using both patch classification metrics and centroid localization metrics, which are furtherly explained in SECTION X. In this sense, the location of the predicted mitosis centroid compared with the location of the original one also gives us information about the model performance during the learning phase, and enables us to use the euclidean distance between both centroids as a parameter to optimize, via the proposed centroid location loss function (SECTION X). Additionally, note that during training, patches that contain mitosis are oversampled to deal with the class imbalance inherent to the mitosis detection task.

\subsubsection{Residual Networks: ResNet18}

The proposed METHOD NAME model is based on a single residual CNN designed for semantic classification of natural images. The residual network comes in a number of different forms, including ResNet16, ResNet18, ResNet34, ResNet50, ResNet101, ResNet110, ResNet152, ResNet164, ResNet1202, and so on. In our case, the chosen configuration was the ResNet18, is a 72-layer architecture with 18 deep layers. This architecture was introduced in 2015 by He et al. \cite{resnet2015}, achieving great performances in different image-related tasks such as classification, localisation, detection and segmentation.

After the first CNN-based design (AlexNet), which won the ImageNet 2012 competition \cite{alexnet2012}, every other winning architecture increased the number of layers in a deep neural network to lower the error rate. This technique is effective for smaller numbers of layers, but when more layers are added, a typical deep learning issue known as the vanishing gradient arises, resulting in the gradient becoming zero or being overly large. Therefore, the training and test error rate similarly increases as the number of layers is increased.

Therefore, the ResNet architecture introduced the idea of Residual Blocks to address the vanishing gradient issue. In their paper, He et al. employed a method known as skip connections in this network. The skip connection bypasses some levels to link layer activations to subsequent layers creating a leftover block. These leftover building blocks are stacked to create resnets. Including this kind of skip connection is that regularisation will skip any layer that degrades architecture performance. As a result, training an extremely deep neural network is possible without encountering issues with vanishing gradients. For the processing of medical pictures, residual networks and their variations have been widely used as the classification backbone. FIGURE X shows the layer architecture of the Resnet18 CNN model.


\subsubsection{Transfer Learning Across Domains}

In order to optimise the vast number of network parameters, deep CNNs training typically demands a large amount of data. Nevertheless, data is typically scarce in medical images, and expert annotation is costly. Therefore, training a deep learning model from scratch for medical image analysis tasks is generally impractical. A widespread solution to overcome this issue is called transfer learning (TL). 

TL with CNNs is the idea that knowledge can be transferred to the parametric model. This means that the learnt CNN parameters for a natural image classification task can be used for a new task in the medical domain. In TL with CNN for medical image classification, in particular, a medical image classification (target task) can be learned by leveraging the generic features learned from the natural image classification (source task) if labels are accessible in both domains. Previous work has been performed in this regard \cite{finetuning_medicalimgs} validating the superiority of pre-trained CNN with adequate fine-tuning, showing the efficacy o transfer learning from the natural image domain to the medical image domain. Herein, we fine-tune the ResNet18 model, which has been pre-trained on the ImageNet \cite{imagenet} natural image classification task. Therefore, we initialise our network with the learnt parameters from the pre-trained model and fine-tune the layers through back-propagation on mitosis data.

\subsubsection{Data Augmentation}

Deep networks typically require a large number of training data to perform effectively. Image augmentation is typically needed to improve the performance of deep networks in order to create a robust image classifier with less training data. Image augmentation artificially generates training images by combining several image processing techniques, such as random rotation, shifts, shear and flips.

There exist different types of image augmentation techniques. The augmentations that remain the pixels’ content unchanged but have variations related to rotations, mirrorings or flips are called spatial augmentations. Also, non-spatial augmentations are the ones that modify the pixels’ information using optical or grid distortions affecting the morphology of the image. Finally, we find the augmentations that affect the pixels’ information but not the image's morphology by varying the image's saturation, contrast, brightness and hue. In our particular case, both spatial and non-spatial image augmentations were applied to the image patches, which consisted of horizontal and vertical flips, random ninety-degree rotations, transposition and both grid and optical distortion.

\subsubsection{Stain Normalization}

In the field of digital pathology, there are very important color and intensity variations in the stainings performed in different laboratories and hospitals. This is critical for the learning of deep neural networks because they need to be trained to be robust against these types of changes in the image properties, as they should be as generalizable as possible to data from other centres.

Stain normalization corresponds to the task of normalizing all the images to the same colour domain before feeding them to the CNN to enable improved quantitative analysis. This consequently increases the prediction accuracy in the validation and test sets, which corresponds to the images that the network has not seen during training. [SHOW FIGURE OF NORMALIZED PATCHES FROM DIFFERENT DOMAINS]. In this work, we performed stain normalization to all the patches involved during training and evaluation using the method proposed by Macenko et al. \cite{macenko_stainnorm}.


\subsection{Centroid Localization Loss}

n this study, we aim to improve both the efficiency of an automatic mitosis detection system by proposing a single-phase model, but also the efficacy of the predictions. Consequently, we introduce an additional term to the binary cross-entropy (BCE) loss which is used during training that leverages the location of the mitosis in the patch. This is the centroid location loss (Lc), which consists of computing the euclidean distance between the pixel that contains the mitosis in the ground truth and the pixel with the maximum probability of containing a mitosis in the class activation map (CAM) of the prediction. This term is added to the BCE Loss together with a regularization term LAMBDA that controls the balance as follows:


$$
L = L_{BCE} + \lambda_{c} L_{C}
$$

$$
L_{BCE} = -\frac{1}{N} \sum_{i=0}^{N} y_{i} \cdot \log \left(\hat{y}_{i}\right)+\left(1-y_{i}\right) \cdot \log \left(1-\hat{y}_{i}\right)
$$


$$
Lc=\sqrt{\sum_{i=1}^{n}\left({c}_\hat{{y}_{i}}-{c}_{{y}_{i}}\right)^{2}}
$$



$$
L = -\frac{1}{N} \sum_{i=0}^{N} y_{i} \cdot \log \left(\hat{y}_{i}\right)+\left(1-y_{i}\right) \cdot \log \left(1-\hat{y}_{i}\right) + \lambda_{c} \sqrt{\sum_{i=1}^{N}\left({c}_\hat{{y}_{i}}-{c}_{{y}_{i}}\right)^{2}}
$$

Introducing this term, to the total loss function, enables us to take into consideration, not only if the patch is classified correctly as having mitosis or not, but also to evaluate how close the prediction is to the actual coordinates of the mitosis in the patch. This technique allows us to benefit from the provided centroid type of data, and therefore, to turn the training into a weakly supervised approach. We optimise the parameters of the METHOD NAME model on mitosis data by minimising the total loss that includes the classification and the location term.

Note that, for simplicity, the patches that contain more than one mitosis inside the patch are discarded for the model training.

